Dialogue Coherence Assessment Without Explicit Dialogue Act Labels

Recent dialogue coherence models use the coherence features designed for monologue texts, e.g. nominal entities, to represent utterances and then explicitly augment them with dialogue-relevant features, e.g., dialogue act labels. It indicates two drawbacks, (a) semantics of utterances is limited to entity mentions, and (b) the performance of coherence models strongly relies on the quality of the input dialogue act labels. We address these issues by introducing a novel approach to dialogue coherence assessment. We use dialogue act prediction as an auxiliary task in a multi-task learning scenario to obtain informative utterance representations for coherence assessment. Our approach alleviates the need for explicit dialogue act labels during evaluation. The results of our experiments show that our model substantially (more than 20 accuracy points) outperforms its strong competitors on the DailyDialogue corpus, and performs on par with them on the SwitchBoard corpus for ranking dialogues concerning their coherence.

==> tex/results.tex <==
\section{Results}  
\label{sec:results}
%
First, we discuss the results for both in problem-domain, and cross problem-domain evaluations.   
%
Then, we evaluate the impact of MTL on the DAP task. 
%
\paragraph{In problem-domain evaluations.} 
%
%
%
Table~\ref{tab:dd_res} shows the accuracy of the baseline models (top) and our model (bottom) for the examined \experiment s on the \dd\ and \sw\ dialogues.  
% 
%

%S-DiCoh
\mbox{\sdicoh} outperforms \random\ and \cosine\ baseline models for all \experiment s on both \dd\ and \sw .
%
This observation confirms the validity of our coherence model where no DA information is taken into account.  
%

\sdicoh\ even achieves the best accuracy for all experiments on \dd\ compared with \aseq\ and \eagrid\ as the baseline models that use DA information. 
%
However, on \sw , \sdicoh\ achieves lower accuracy than \aseq\ and \eagrid\ for all \experiment s except \uishort . 
% 
Note that unlike \eagrid\ and \aseq , \sdicoh\ is completely agnostic to DA information. 

%
%M-DiCoh
\mdicoh\ substantially outperforms \random\ and \cosine\ (which do not use DAs) for all \experiment s on both \dd\ and \sw. 
%
As \mdicoh\ also outperforms \sdicoh\ for all \experiment s on both corpora, we conclude that 
our proposed MTL approach effectively uses DA information to enrich utterance vectors for dialogue coherence assessment. 

Compared with \aseq\ and \eagrid , our \mdicoh\ achieves the highest accuracy for all \experiment s on \dd, showing that our approach for involving DAs yields more informative utterance representations for coherence assessments. 
%
However, on \sw , \mdicoh\ increases the accuracy of \sdicoh\ up to those of \eagrid\ for \uoshort\ and \huoshort.    
%
Surprisingly, it achieves lower accuracy than \eagrid\ for \urshort.  
% 
% 

We speculate that the reason that \mdicoh\ outperforms \aseq\ and \eagrid\ on \dd\ but not on \sw\ is because the \aseq\ and \eagrid\ models explicitly use \emph{gold} DA labels during evaluation but \mdicoh\ does not; and the DA \annotation s in \sw\ are about $10$ times higher fine-grained than those in \dd\ (see Table~\ref{tab:datasets}).
%
This interpretation becomes more obvious by observing a considerable drop in the performance of \aseq\ and \eagrid\ when they are evaluated on \dd\ compared with when they are evaluated on \sw.
%
In contrast, our \mdicoh, which uses DAs only during training to obtain better utterance vectors, performs almost evenly on both corpora. 
%
%
Since our model does not need any DA labels during evaluation, it is more suitable for evaluating dialogue coherence in real scenarios compared with the examined models.   
% 

%
\pgfplotstableread[row sep=\\,col sep=&]{
testset  &  MDiCoh &  EAGrid\\
UO  & 95.92 & 71.72 \\ 		
UI	& 84.46 & 57.65 \\ 
UR	& 74.44 & 57.10 \\ 
EUO & 87.84 & 66.93 \\ 
    }\uo
\pgfplotstableread[row sep=\\,col sep=&]{
testset & MDiCoh &  EAGrid\\
UO  & 95.04 & 65.51\\
UI	& 88.20 & 60.93 \\ 
UR	& 74.91 & 55.59 \\ 
EUO & 85.24	& 65.33 \\ 
    }\ui
\pgfplotstableread[row sep=\\,col sep=&]{
testset  &  MDiCoh &  EAGrid\\
UO  & 92.75 & 58.70  \\
UI	& 82.14 & 52.65	\\ 		
UR	& 83.02 & 68.49	\\
EUO & 85.27 & 57.95	\\ 
    }\ur
\pgfplotstableread[row sep=\\,col sep=&]{
testset  &  MDiCoh &  EAGrid\\
UO  & 94.4 & 67.41 \\
UI	& 81.33 & 57.53 \\ 
UR	& 73.02 & 54.95 \\ 
EUO & 88.55 & 67.18 \\ 
    }\euo

\begin{figure*}[!ht]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccc@{}}
\begin{tikzpicture}
            \begin{axis}[
                    ybar,
                    bar width=5mm,
                    height=12cm,
                    legend style={at={(0.5,1.0)}, anchor=north,legend columns=-1,
                    font=\LARGE},
                    symbolic x coords={UO,UI,UR,EUO},
                    xtick=data,
                    nodes near coords,
                    every node near coord/.append style={rotate=90, anchor=west, font=\huge},
                    ymin=50,ymax=100,
                    ylabel={Acc (\%)},
                    ticklabel style= {font=\huge},
                    ylabel style={font=\huge}
                ]
                
        \addplot[fill=white] table[x=testset,y=MDiCoh]{\uo};
        \addplot[fill=black] table[x=testset,y=EAGrid]{\uo};
        \legend{MDiCoh, EAGrid};
        \end{axis};
        \end{tikzpicture}
         &
        \begin{tikzpicture}
            \begin{axis}[
                    ybar,
                    bar width=5mm,
                    %width=10cm,
                    height=12cm,
                    legend style={at={(0.5,1.0)}, anchor=north,legend columns=-1, font=\LARGE},
                    symbolic x coords={UO,UI,UR,EUO},
                    xtick=data,
                    nodes near coords,
                    every node near coord/.append style={rotate=90, anchor=west, font=\huge},
                    ymin=50,ymax=100,
                    ylabel={Acc (\%)},
                    ticklabel style= {font=\huge},
                    ylabel style={font=\huge}
                ]
        \addplot[fill=white] table[x=testset,y=MDiCoh]{\ui};
        \addplot[fill=black] table[x=testset,y=EAGrid]{\ui};
        \legend{MDiCoh, EAGrid};
        \end{axis}
        \end{tikzpicture}
         &
        \begin{tikzpicture}
            \begin{axis}[
                    ybar,
                    bar width=5mm,
                    %width=10cm,
                    height=12cm,
                    legend style={at={(0.5,1.0)}, anchor=north,legend columns=-1, font=\LARGE},
                    symbolic x coords={UO,UI,UR,EUO},
                    xtick=data,
                    nodes near coords,
                    every node near coord/.append style={rotate=90, anchor=west, font=\huge},
                    ymin=50,ymax=100,
                    ylabel={Acc (\%)},
                    ticklabel style= {font=\huge},
                    ylabel style={font=\huge}
                ]
        \addplot[fill=white] table[x=testset,y=MDiCoh]{\ur};
        \addplot[fill=black] table[x=testset,y=EAGrid]{\ur};
        \legend{MDiCoh, EAGrid};
        \end{axis}
        \end{tikzpicture}
         
         &
        \begin{tikzpicture}
            \begin{axis}[
                    ybar,
                    bar width=5mm,
                    %width=10cm,
                    height=12cm,
                    legend style={at={(0.5,1.0)}, anchor=north,legend columns=-1, font=\LARGE},
                    symbolic x coords={UO,UI,UR,EUO},
                    xtick=data,
                    nodes near coords,
                    every node near coord/.append style={rotate=90, anchor=west, font=\huge},
                    ymin=50,ymax=100,
                    ylabel={Acc (\%)},
                    ticklabel style= {font=\huge},
                    ylabel style={font=\huge}
                ]
        \addplot[fill=white] table[x=testset,y=MDiCoh]{\euo};
        \addplot[fill=black] table[x=testset,y=EAGrid]{\euo};
        \legend{MDiCoh, EAGrid};
        \end{axis}
        \end{tikzpicture}
         
         \\
         \huge{(a) \uoshort}
         &
         \huge{(b) \uishort}
         &
         \huge{(c) \urshort}
         &
         \huge{(d) \huoshort}
 \end{tabular}
 }
    \caption{Comparing \eagrid\ (black bars) and \mdicoh\ (white bars) in cross problem-domain. 
    The labels of figures are the perturbations of the training sets
    and the labels on x-axes are the perturbations of the test sets.}
    \label{fig:ext_results}
    
\end{figure*}

%
%
To shed some lights on which parts of a dialogue receive higher attention in our model for assessing the coherence of the dialogue, we analyze the attention weights. 
%
As an example, Table~\ref{tab:attention} illustrates the attention values for an example dialogue from \dd. 
%

\begin{table}[!ht]
    \small
    \centering
    \begin{tabular}{l}
        \toprule
         \textcolor{black!50}{hello} \textcolor{black!50}{,} \textcolor{black!50}{where} \textcolor{black!50}{can} \textcolor{black!50}{i}  \textcolor{black!50}{buy} \textcolor{black!50}{an} \textcolor{black!50}{inexpensive} \textcolor{black!50}{cashmere} \textcolor{black!50}{sweater} \textcolor{black!50}{?} \\
         \textcolor{black!50}{maybe} \textcolor{black!50}{you} \textcolor{black!50}{should} \textcolor{black!50}{look} \textcolor{black!50}{around} \textcolor{black!50}{for} \textcolor{black!50}{an} \textcolor{black!50}{outlet} \textcolor{black!50}{.} \\
         \textcolor{black!50}{that} \textcolor{black!50}{is} \textcolor{black!50}{a} \textcolor{black!50}{wonderful} \textcolor{black!50}{idea} \textcolor{black!50}{.} \\
         \textcolor{black!50}{outlets} \textcolor{black!50}{have} \textcolor{black!50}{more} \textcolor{black!50}{reasonable} \textcolor{black!50}{prices} \textcolor{black!50}{.} \\
         \textcolor{black!50}{no problem} \textcolor{black!50}{.} \textcolor{black!50}{good} \textcolor{black!50}{luck} \textcolor{black!50}{.}\\
        \bottomrule
         
    \end{tabular}
    \caption{An illustration of attention distributions over words in a dialogue from \dd. Different gray shades show different attention weights.}
    \label{tab:attention}
\end{table}
%
We observe that the model assigns higher attention values to wh-questions, adjectives and adverbs in a question utterance. 
%
While for other utterances, it mostly focuses on nouns, considering their semantic relationships, e.g., \emph{outlet}, \emph{inexpensive}, \emph{prices}.  
%


\paragraph{Cross problem-domain evaluations.}
%
Here, we compare \eagrid\ and \mdicoh\ for the cross problem-domain evaluations on \dd, where the best performing model trained on the training set of one \experiment\ is evaluated on each of the test sets of other \experiment s. 
% 
Therefore, the perturbation methods used for constructing the training sets differ from those used for creating the test sets. 
%
Figure~\ref{fig:ext_results} shows the results on the test sets of the \experiment s, where the models are trained on the training set created by the (a) \uoshort, (b) \uishort, (c) \urshort, and (d) \huoshort\  perturbations. 
%

%
For all perturbations used to construct the training sets, we observe that \mdicoh\ outperforms \eagrid\ for all test perturbations.  
% 
%
Interestingly, among all test perturbations, both \mdicoh\ and \eagrid\ achieve the highest accuracy on \uoshort, which can be because this perturbation perturbs the whole dialogue and consequently is easier to learn than other perturbations. 
%
A similar behaviour has been reported by \newcite{cervone18}. 
%

 
\paragraph{The impact of our MTL on the DAP model} 
%
Since using DAP as an auxiliary task improves the performance of our coherence model; in the following experiment, we investigate the impact of MTL on the DAP task. 
%
We train our DAP model without any coherence supervision signal, S-DAP, with $\mathcal{L}=\frac{\mathcal{L}^{dial_i}_{da} + \mathcal{L}^{dial_j}_{da}}{2}$ in Equation~\ref{eq:total_loss}, and compare it with the model that is trained with our MTL, M-DAP. 

Table~\ref{tab:da_dd} shows the F1 metric\footnote{We use F1 because there are more than two DA labels.} of these models for our \experiment s on \dd. 
%
\begin{table}[!ht]
    \small
    \centering
    \begin{tabular}{lcccc}
        \toprule
                     & \uoshort & \uishort & \urshort & \huoshort \\
        \midrule
        SVM-BoW    & 76.11    &  75.52 & 74.49 & 75.73 \\ 
        \midrule
        S-DAP       & 78.96&  79.25 & 79.28&  79.29\\ 
        M-DAP       & 77.90& 78.44& 77.08 & 78.97\\
        \bottomrule
    \end{tabular}
    \caption{The  F1 metric of the DAP model for the test sets of the \experiment s on \dd.  
    S-DAP is the model trained without any coherence supervision, and M-DAP is the model trained with MTL.} 
    \label{tab:da_dd}
\end{table}
%
We use SVM supplied with \mbox{Bag-of-Word} utterance representations as baseline to put our results in context. 
%
We notice that our DAP model performs slightly worse when MTL is used for training. 
%
However, the main goal of this paper is to use DAP to obtain more informative utterance vectors for coherence assessment, and remove the need for DA labels during evaluation. 
Although improving the performance of the DAP model could be a possible future work, it is out of the scope of this paper.  
%
